Blocked All-Pairs Shortest Paths Algorithm on Intel Xeon Phi KNL Processor: A Case Study

Manycores are consolidating in HPC community as a way of improving performance while keeping power efficiency. Knights Landing is the recently released second generation of Intel Xeon Phi architecture. While optimizing applications on CPUs, GPUs and first Xeon Phi's has been largely studied in the last years, the new features in Knights Landing processors require the revision of programming and optimization techniques for these devices. In this work, we selected the Floyd-Warshall algorithm as a representative case study of graph and memory-bound applications. Starting from the default serial version, we show how data, thread and compiler level optimizations help the parallel implementation to reach 338 GFLOPS.

==> alg1.tex <==
\begin{algorithm}[hb!]
\caption{Naive Floyd-Warshall Algorithm}\label{alg:floyd_naive}
	\begin{algorithmic}[1]
		%\State \Comment {$numSequences$ is the number of database sequences}
		%\State \Comment{$t$ is the number of threads}		
		\For{$k = 0..N$} 
			\For{$i = 0..N $} 
				\For{$j = 0..N $} 
					\If{$D_{i,k} + D_{k,j} < D_{i,j}$}
						\State{$D_{i,j} = D_{i,k} + D_{k,j}$}
						\State{$P_{i,j} = k$}
					\EndIf
				\EndFor
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


==> alg2.tex <==
\begin{algorithm}[hb]
\fontsize{8}{12}
%\algsetup{linenosize=\tiny}
\caption{Blocked Floyd-Warshall Algorithm}\label{alg:floyd_blocked}
 \begin{multicols}{2}
	\begin{algorithmic}[1]
		%\State \Comment {$numSequences$ is the number of database sequences}
		%\State \Comment{$t$ is the number of threads}		
	\Function{UPDATE}{$B^1$,$B^2$,$B^3$,$P$,base}		
		\For{$k = 0..BS$} 
			\For{$i = 0..BS $} 
				\For{$j = 0..BS $} 
					\If{$B^2_{i,k} + B^3_{k,j} < B^1_{i,j}$}
						\State{$B^1_{i,j} = B^2_{i,k} + B^3_{k,j}$}
						\State{$P_{i,j} =$ base+$k$}
					\EndIf
				\EndFor
			\EndFor
		\EndFor
	\EndFunction
	\State
	\State
	\State		
	\For{$k = 1..S$}
		\State {base = $k \times BS$}
		\State \Comment {Phase 1}
		\State {UPDATE($B_{k,k}$,$B_{k,k}$,$B_{k,k}$,$P_{k,k}$,base)}		
		\State 		\Comment {Phase 2}		
		\For{$j = 1..B; j \neq k$}
			\State {UPDATE($B_{k,j}$,$B_{k,k}$,$B_{k,j}$,$P_{k,j}$,base)}
		\EndFor
		\State \Comment {Phase 3}		
		\For{$i = 1..B; i \neq k$}		
			\State {UPDATE($B_{i,k}$,$B_{i,k}$,$B_{k,k}$,$P_{i,k}$,base)}
		\EndFor
		\State \Comment {Phase 4}	
		\For{$i,j = 1..B; i,j \neq k$}					
			\State {UPDATE($B_{i,j}$,$B_{i,k}$,$B_{k,j}$,$P_{i,j}$,base)}
		\EndFor		
	\EndFor

	\end{algorithmic}
\end{multicols}
\end{algorithm}

